Exact Acceleration of Subgraph Graph Neural Networks by Eliminating Computation Redundancy

Graph neural networks (GNNs) have become a prevalent framework for graph tasks. Many recent studies have proposed the use of graph convolution methods over the numerous subgraphs of each graph, a concept known as subgraph graph neural networks (subgraph GNNs), to enhance GNNs' ability to distinguish non-isomorphic graphs. To maximize the expressiveness, subgraph GNNs often require each subgraph to have equal size to the original graph. Despite their impressive performance, subgraph GNNs face challenges due to the vast number and large size of subgraphs which lead to a surge in training data, resulting in both storage and computational inefficiencies. In response to this problem, this paper introduces Ego-Nets-Fit-All (ENFA), a model that uniformly takes the smaller ego nets as subgraphs, thereby providing greater storage and computational efficiency, while at the same time guarantees identical outputs to the original subgraph GNNs even taking the whole graph as subgraphs. The key is to identify and eliminate the redundant computation among subgraphs. For example, a node $v_i$ may appear in multiple subgraphs but is far away from all of their centers (the unsymmetric part between subgraphs). Therefore, its first few rounds of message passing within each subgraph can be computed once in the original graph instead of being computed multiple times within each subgraph. Such strategy enables our ENFA to accelerate subgraph GNNs in an exact way, unlike previous sampling approaches that often lose the performance. Extensive experiments across various datasets reveal that compared with the conventional subgraph GNNs, ENFA can reduce storage space by 29.0% to 84.5% and improve training efficiency by up to 1.66x.

==> 9_rebuttal.tex <==
\section{R1}
\stitle{Experimental Settings.}
The experimental setup is poorly described. It’s unclear what the baseline comparisons entail and how many layers were used.

\stitle{Other baselines.}
Only compares against a single baseline (ESAN), which may not provide a comprehensive evaluation of the framework’s effectiveness.

\stitle{pivot nodes and hops memory}
Identifying pivot nodes and hops requires additional memory and computation, which the experiments do not seem to account for.


Thanks for your insightful comments. Our responses to the reviewer's concerns are as follows.

1. Experimental setup poorly described.

In storage consumption experiments, subgraph GNNs generate and store all duplicate graphs. This process is not dependent on the number of MPNN layers.
Thus, in Figure 4/6, we report one bar for baseline of each policy since a subgraph GNN with either layer produces the same result.
Regarding time cost, we vary the number of layers for both ENFA and the baseline for pair comparison.
In the revision, we plan to provide a more detailed explanation of our experimental setups.

2. Comparison with a single baseline.

While we validates ENFA whthin the ESAN framework, the variant policies tested in our experiments encompass a range of recent works. Aside from the node-deleting and edge-deleting policies in ESAN, we also test the node-marking policy studied in [1][2].
The tested variant of subgraph GNNs, i.e. those with subgraph message passings, have also been employed in [3][4].
We believe ENFA could be applicable to a broad spectrum of previous works. In our revision, we will provide a clearer description of the roles these works play in our evaluation.

[1] Identity-aware graph neural networks.

[2] A Complete Expressiveness Hierarchy for Subgraph GNNs via Subgraph Weisfeiler-Lehman Tests.

[3] From Stars to Subgraphs: Uplifting Any GNN with Local Structure Awareness.

[4] Understanding and extending subgraph gnns by rethinking their symmetries.

3. Memory and computation of pivot nodes and hops.

We apologize for the ambiguity in our discussion of pivot nodes. We have indeed demonstrated the memory consumption of pivot nodes and hops in our evaluation in Figure 6 where the yellow part denotes the proportion of pivot nodes and hops occupied. By sacrificing storage for pivot hops and nodes, ENFA significantly shrinks the size of the stored graphs (blue part).

As for time cost, pivot nodes and hops have a distinctive feature: they are irrelevant to the input of models. This information can be pre-computed during the process of duplicating graphs for subgraph GNNs and the pre-computation time is minimal compared to the training time of subgraph GNNs.
For PROTEINS dataset, it takes less than 20 seconds to duplicate the graphs and compute the pivot hops, while training a subgraph GNN takes up to 350 seconds. The time cost is slight and does not affect the training process. We plan to add this description in our revision.

\section{R2}
\stitle{Expressive claim.}
The claim in the abstract "To maximize the expressiveness, subgraph GNNs often require each subgraph to have equal size to the original graph" is not clear - do the authors refer to node marking specifically? this isn't correct for ego-net encoding for example.

\stitle{Baseline claim.}
It is not clear what is the baseline followed in the experiments. I suggest that the authors add it to the cpation of the figures and elaborate in text as well.

\stitle{ENFA cost most time.}
It seems like in practice, the method take the same or more time in many cases, probably due to the mechanism that checks whether computations are redundant or not. This makes the method less practical.

\stitle{how this works can be utilized in ego-nets}
It is not clear how this method can be used for strong encodings like ego-networks.

\stitle{Larger graphs}
The graphs used in this paper are somewhat small. I think that given that, there is usually not much of a memory problem but rather time, which as shown in the paper is in many cases the same runtime as with baseline subgraph GNNs. I think that results on large scale graphs would be more convincing as a use case of the method.

\stitle{Related work discussion.}
Missing discussion of a recent light weight subgraph GNNs - "Efficient Subgraph GNNs by Learning Effective Selection Policies".


Thanks for your insightful comments. Our responses to the reviewer's concerns are as follows.

1. Unclear expressive claim.

Our statement relies on the theoretical results in [1], which indicate a subgraph GNN with the node marking policy achieves the maximum expressiveness among all subgraph GNNs, including those with the ego-net policy. Thus, subgraph GNNs with subgraphs of the same size as the original graphs play a crucial role.
In our revised version, we will present a more explicit claim concerning expressiveness.

2. Unclear baseline elaboration.

We appreciate your suggestion and will explicitly name the baseline, i.e., ESAN, in our revised version.

3. Inferior time cost of ENFA.

Apologizes if the running time figures caused confusion. Generally, ENFA outperforms the baseline in most cases.
Figure 5 may caused confusion due to limited space, as we report the results of two policies in each figure. Two lines with the same color should be comparable, as they represent ENFA and the baseline with the same policy. This comparison demonstrates the time ENFA could save while ensuring the exact acceleration.
ENFA shows considerably less time cost in most cases.
For example, ENFA could save more than 20%
time in 48 cases out of 64 cases in Figure 5, and the largest speedup reaches 1.66x on Peptides-func dataset.

4. Utilization in ego-nets.
As discussed in the Appendix, ENFA can be utilized for subgraph GNNs with ego-net policy by identifying boundary nodes of ego-nets as pivot nodes. However, it may not gain advantage as ENFA also makes message passing on ego nets.
On the other hand, recent studies[1] show that the policies with subgraphs the same size as the original graphs obtain the maximum expressiveness among all policies. ENFA shows that we can extract exact output as subgraph GNNs with the maximum expressiveness by making massage passing on smaller graphs, i.e., the ego nets.

5. Larger graphs for evaluation.
We kindly claim that our evaluation includes datasets that cover a wide range of graph sizes. This paper focuses on subgraph GNNs, which are mainly used on graph classification and regression tasks. These tasks usually involve graphs with a size not exceeding 200. The Peptides-func dataset in our evaluation contains an average graph size of 150, which is larger than most of the graph classification tasks.

6. Importance of memory consumption.
We respectfully disagree with your viewpoint.
Memory consumption is a severe issue due to the design of subgraph GNNs, which require duplicating a large number of graphs for training. This process results in dramatic increase storage both on hard  disks (before training) and GPU (while training).
As shown in Table 1, datasets explode hundreds of times after the pre-computation of subgraph GNNs.
Besides, the Peptides dataset exploded to 35GB, although its original size was 752MB.

6. Lacking of related works.
We appreciate your suggestion and will discuss the proposed paper in the revision.
The paper employs sampling strategies to reduce the number of subgraphs. As discussed in our Appendix (Subgraph GNNs with Subsampling Strategies), such a strategy affects the output of subgraph GNNs, making their performance unpredictable. Conversely, ENFA guarantees exact output as any subgraph GNNs, and could also be applied to the sampled subgraphs to obtain the output efficiently. 

[1] A Complete Expressiveness Hierarchy for Subgraph GNNs via Subgraph Weisfeiler-Lehman Tests. In ICML.

NEW: 

Thanks for your insightful comments. Our responses are as follows.

1. Unclear expressive claim.

Our statement relies on the theoretical results [1], which indicate a subgraph GNN with the node marking policy achieves the maximum expressiveness among all subgraph GNNs, including those with ego-net policy. Thus, subgraph GNNs with the same size as the original graphs play a crucial role and become our focus.

2. Baseline elaboration.

We will explicitly name the baseline in our revision.

3. Inferior time cost of ENFA.

We would like to emphasize that ENFA generally outperforms the baseline in all cases. In Figure 5, due to limited space, we report the results of two policies in each figure. It's important to clarify that two lines of the same color are comparable, as they represent the results with the same policy.

4. Utilization in ego-nets.

As discussed in appendix, ENFA can be utilized for subgraph GNNs with ego-net policy by identifying boundary nodes of ego-nets as pivot nodes. However, ENFA may not gain advantage on ego-nets. Following the expresiveness statement in 1, ENFA shows that we can extract exact output as subgraph GNNs with the maximum expressiveness by smaller graphs.

5-1. Larger graphs for evaluation.

We kindly claim that our evaluation covers graphs with a wide range of sizes. Subgraph GNNs are mainly used on graph classification tasks, where the graph sizes generally do not exceed 300. The Peptides-func dataset in evaluation contains an average graph size of 150, larger than a majority of graph classification tasks in practice.

5-2. Importance of memory consumption.

We kindly emphasize that memory consumption is a severe issue due to design of subgraph GNNs, which requires duplicating a large number of graphs for training. This process results in dramatic increase storage both on hard disks and GPU. The datasets in Table 1 explode hundreds of times after the pre-computation of subgraph GNNs. Besides, the Peptides dataset exploded to 35GB, although its original size was 752MB.

6. Lacking of related works.

We will discuss the paper, which reduces number of subgraphs by samplings, in the revision. As discussed in appendix, samplings affect the output of subgraph GNNs, making their performance unpredictable. Conversely, ENFA guarantees exact output and can also be applied to the sampled subgraphs to obtain the output efficiently. 

[1] A Complete Expressiveness Hierarchy for Subgraph GNNs via Subgraph Weisfeiler-Lehman Tests.

\section{R3}
\stitle{Structure of the paper.}
the abstract could say directly that node deletion and node marking are common to generate the subgraphs and then say that this implies redundant computation. It took me too long to understand the setting/problem that the paper is solving.

The intro has the same problem as the abstract: make more clear how a subgraph GNN works. The subgraphs are definitely not "rooted" as this would imply some kind of directedness and is only simple in trees.

\stitle{on GCN}
the authors did experiments on GIN, silently ignoring that GCN would not work here (due to the sqrt(D) operation on top of simple message passing)

\stitle{Equations.}
Preliminaries: I prefer it if most uncommon operators are defined above the equation and not (far) below. (eq1)

\stitle{Complexity.}
the complexity part is not great, especially the bounded degree assumption only holds for molecule graphs, but definitely not for social networks.

the whole complexity analysis hinges on constant d, this should be more prominent.

\stitle{Larger layers.}
It is not uncommon to train 10 layer GNNs (maybe not subgraph GNNs, but normal ones). Still finite, but much larger than in this paper.



\stitle{Virtual nodes.}
a remark on Virtual nodes would also be in order - as those are not supported (instead one can use subgraph message passing)

\stitle{Related works.}
related work missed AdaptGear (2023) as an example for making GNNs fast.

\stitle{Figure 6}
Figure 6 is confusing: how many layers does the baseline have and why not pair them with differently deep ENFA models?

\stitle{Other questions.}
Lehman -> Leman (as in the citation)

use booktabs for all tables. They look so much better that way. (The current tables in the paper are quite ugly tbh)

Figure 1 had me confused at first (mostly because I only worked with subgraph GNNs with the node-delete policy) and its not as clear what is happening here.

Please use \\operatorname in eq2 for all operators

Please abbreviate equations as Eq 1 and not Equ 1 (I have never seen the latter and the latex package cleverref also does not do that)

Thanks for your constructive comments. We address the
reviewer's concerns are as follows.

1. Applying ENFA on GCN layers.

The proposed method could be applied to other MPNN layers relying on degrees, like GCN, and we have reported the experimental results on GCN layers in the appendix.

i. The nodes on the boundary of the generated ego nets in ENFA have their degrees changed compared to the original graphs. We could solve this issue by generating a larger ego net. In other words, if a subgraph GNN contains $L$ MPNN layers, we generate an $L+2$-hop ego net from the marked/deleted nodes.
Thus, all nodes with no greater than $L$ hops to the marked/deleted nodes have themselves and their neighbors containing degrees the same as that in the original graphs.
% In our experiments, ENFA always generates the $L+2$-hop ego nets for a subgraph GNN with $L$ layers.

ii. Figure 9 in the Appendix reports the experimental results on GCN and GraphConv layers. For datasets ogbg-molhiv, ogbg-moltox21, ENFA and the baseline with GCN layers show similar trends compared to those with GCN layers.
However, the time and gap between ENFA and the baseline significantly increase for the Peptides-func dataset. This is attributed to large graph size in Peptides-fun, making the computation of $D^{{1/2}}AD^{{1/2}}$ more time-consuming.

2. Structure of the paper.

Thanks for your constructive suggestion. We will employ a more succinct way to motivate our paper and introduce the proposed method in our revision.

3. Complexity analysis.
Thanks for your suggestion. We will reserve the constant $d$ in our complexity analysis in the revision.

4. ENFA with more layers.
The five datasets except for Peptides-func have small diameters close to 10. This indicates that ENFA cannot show advance on these datasets as an ego net with 10 hops will almost cover the whole graphs.
We will try ENFA with 10 layers on Peptides-func to show its scalability in our revision.

5. Application to virtual nodes.
Thanks for your suggestion. We will add a discussion on virtual nodes in our revision.

6. Baseline report in storage consumption.
For conventional subgraph GNNs with original graphs, although their training time is affected by the number of layers, it occupies the same space for different numbers of layers, as the whole graphs should always be stored. Thus, only one bar is reported in the experiments of storage, including Figure 4 and Figure 6.

7. Missing related works.

Thanks for your suggestion. We will supplement related references in our revision.

3. Other formalism problems.

Thanks for your constructive suggestion. We will correct these issues in our revision.


NEW:

Thanks for your insightful comments. Our responses are as follows.

1. Applying ENFA on GCN layers.
The proposed method can indeed be applied to other MPNN layers relying on degrees, like GCN. We have included the experimental results on GCN layers in the appendix.
(i). The nodes on the boundary of the generated ego nets in ENFA have their degrees changed. This issue can be solved by generating larger ego nets. For a subgraph GNN with $L$ MPNN layers, we generate an (L+2)-hop ego net from the marked/deleted nodes.
This ensures that all nodes, which are no more than $L$ hops to the marked/deleted nodes, and their neighbors, retain their original degrees.
(ii). Figure 9 in the Appendix reports the experimental results on GCN and GraphConv layers. For the ogbg-molhiv and ogbg-moltox21 datasets, With GCN layers, ENFA shows similar results compared to those with GIN layers. However, the time of and gap between ENFA and the baseline significantly increase for the Peptides-func dataset, largely due to the larger graph size which makes the computation of $D^{{1/2}}AD^{{1/2}}$ more time-consuming.

2. Structure of the paper.
We appreciate your suggestion. In our revision, we will aim to present a more concise motivation for our paper and a clearer introduction to the proposed method.

3. Complexity analysis.
Upon your recommendation, we will reserve the constant $d$ in our complexity analysis in the revision.

4. ENFA with more layers.
Since the five datasets except for Peptides-func have small diameters close to 10, ENFA cannot show significant improvement as an 10-hop ego net will almost cover the entire graphs.
We will try ENFA with 10 layers on Peptides-func dataset to show ENFA's scalability in our revision.

5. Application to virtual nodes.
Thanks for your suggestion. We will include a discussion on virtual nodes in our revised version.

6. Baseline report in storage consumption.
Conventional subgraph GNNs with original graphs occupy the same storage space for different numbers of layers, as the whole graphs should always be stored, even though their training time is affected by the number of layers. Therefore, only one bar is reported in the storage consumption experiments, including Figure 4 and Figure 6.

7. Missing related works and other formalism problems.
We appreciate your constructive feedback and will include additional related references and rectify these issues in our revised version.


\section{SPC}
We thank all reviewers and 
We would like to draw your attention to reviewer sRVn's weaknesses 3 and 5, regarding the time efficiency of ENFA and the size of the graphs used in our study.

Regarding weakness 3, the reviewer posits that our proposed method takes the same or more time in many cases. However, this is contrary to our findings, as depicted in Figure 5, where ENFA consistently exhibits considerably less time consumption compared to the baseline.

Regarding weakness 5, the reviewer suggests that the graph sizes used in our evaluation are relatively small. Nevertheless, in the context of graph classification and graph regression tasks, where subgraph GNNs are primarily applied, the majority of datasets typically range from tens to 200-300 nodes, with the aim being to predict the property of each graph.
In our study, we utilized the Peptides-func dataset, which contains an average of approximately 150 nodes and 300 edges. This is representative of the majority of datasets typically used in practical graph classification tasks.


==> checklist.tex <==
\vspace{-4pt}
\section{Reproducibility Checklist}
This paper:
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) {\bf Yes}
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) {\bf Yes}
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) {\bf Yes}
\end{itemize}

\noindent Does this paper make theoretical contributions? (yes/no) {\bf Yes}

\noindent If yes, please complete the list below.
\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no) {\bf Yes}
\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no) {\bf Yes}
\item Proofs of all novel claims are included. (yes/partial/no) {\bf Yes}
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no) {\bf Yes}
\item Appropriate citations to theoretical tools used are given. (yes/partial/no) {\bf Yes}
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA) {\bf Yes}
\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA) {\bf Yes}
\end{itemize}

\noindent Does this paper rely on one or more datasets? (yes/no) {\bf Yes}

\noindent If yes, please complete the list below.
\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) {\bf Yes}
\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) {\bf NA}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) {\bf NA}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) {\bf Yes}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) {\bf Yes}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) {\bf Yes}
\end{itemize}

\noindent Does this paper include computational experiments? (yes/no) {\bf Yes}

\noindent If yes, please complete the list below.
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (yes/partial/no) {\bf Yes}
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) {\bf Yes}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) {\bf Yes}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) {\bf Yes}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) {\bf Yes}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) {\bf Yes}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) {\bf Yes}
\item This paper states the number of algorithm runs used to compute each reported result. (yes/no) {\bf Yes}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) {\bf Yes}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) {\bf Yes}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) {\bf Yes}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) {\bf Yes}
\end{itemize}
